LookAhead: Augmenting Crowdsourced Website Reputation Systems With Predictive Modeling

Unsafe websites consist of malicious as well as inappropriate sites, such as those hosting questionable or offensive content. Website reputation systems are intended to help ordinary users steer away from these unsafe sites. However, the process of assigning safety ratings for websites typically involves humans. Consequently it is time consuming, costly and not scalable. This has resulted in two major problems: (i) a significant proportion of the web space remains unrated and (ii) there is an unacceptable time lag before new websites are rated. In this paper, we show that by leveraging structural and content-based properties of websites, it is possible to reliably and efficiently predict their safety ratings, thereby mitigating both problems. We demonstrate the effectiveness of our approach using four datasets of up to 90,000 websites. We use ratings from Web of Trust (WOT), a popular crowdsourced web reputation system, as ground truth. We propose a novel ensemble classification technique that makes opportunistic use of available structural and content properties of webpages to predict their eventual ratings in two dimensions used by WOT: trustworthiness and child safety. Ours is the first classification system to predict such subjective ratings and the same approach works equally well in identifying malicious websites. Across all datasets, our classification performs well with average F$_1$-score in the 74--90\% range.

==> conclusions.tex <==
\section{Conclusions}
In this paper we present LookAhead...
We show that...

To our knowledge this is...


==> contentFeatures.tex <==
%!TEX root = ../submission.tex

\section{Augmenting Prediction with Content-based Features}
\label{sec:content}

\subsection{Towards Content-based Features}


Towards capturing the content related properties, we propose the use of features extracted from the embedded (forward) links of web pages. To gain further insights into the thematic content, we also propose the use of a topic model-based feature-set. In the following we describe each type of features in detail.

\subsubsection{Embedded Link-based Features} 
\label{sssec:ecdf}
In trying to extract a simple yet effective clues about the content
of a web page, we hypothesize that the content of a page is related to
the content of the pages it links to. 
\ifsubmission
\else
In other words, we make use of the hypothesis: ``{\em You are the company you
keep}". This saying is based on the fact that often knowledge about a unknown person's friends provides some idea about the person itself, e.g, the person's interests or personality can be guessed.
\fi
Very similar ideas has been successfully applied in the field of collaborative-filtering to recommend products to a person based on the interests of people similar to him~\cite{breese98empirical}. 
\ifsubmission
\else
Recently, Truong et al.~\cite{truong14company} have successfully applied the same hypothesis in predicting malware infection susceptibility of a mobile device just by looking at the set of applications running on the device.
\fi

\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{pics/linkFeatureOverview}
\caption{Overview of the embedded link-based feature extraction procedure. For a given webpage (on the left), we identify the set of out going web links (in the middle) present on the page and fetch the reputation ratings of those embedded links. We use the reputation ratings to compute an empirical cumulative distribution function (ECDF).}
\label{fig:ecdfOverview}
\end{figure}
 

In case of web pages, the hypothesis can be easily conceptualized. For example, often a web page contains a set of links to other web pages and reputation ratings of the linked web pages can be used to extract important clues about the content safety of the web page under consideration. Building on this idea, we propose a features extraction scheme utilizing the available reputation ratings of the embedded links. Interestingly, the number of web links embedded in an arbitrary web page tend to vary significantly, e.g., web pages may contain an arbitrary number of embedded links, e.g., the number can vary between zero and a very large number (few hundreds). Moreover, the range of the reputation ratings can be arbitrary. Thus, a novel feature extraction scheme is needed that can handle the arbitrary number of links, at the same time it is less sensitive to the arbitrary ranges of the reputation ratings. 

\begin{figure*}
\centerline{
	\subfigure[Histogram showing the frequency distribution of reputation ratings of embedded web links found within a web page.]{
	\label{fig:framework:1st}
	\includegraphics[width=0.3\linewidth]{pics/histRS}\label{fig:histRS}}
	\subfigure[Empirical Cumulating Distribution Function (ECDF) computed from the reputation ratings.]{
	\label{fig:framework:2nd}	
	\includegraphics[width=0.3\linewidth]{pics/ecdfExample}\label{fig:ecdfExample}}
	\subfigure[The ECDF-based features by computing the inverse.]{
	\label{fig:framework:1st}
	\includegraphics[width=0.292\linewidth]{pics/ecdfFeatures}\label{fig:ecdfFeatures}}
	}
\caption{Exemplary illustration of (a) the distribution of reputation ratings, (b) their Empirical Cumulative Distribution Function, and (c) ECDF-based features.}
\label{fig:rsDistribution}
\end{figure*}


Empirical cumulative distribution function (ECDF)-based feature extraction has been previously explored in the field of ubiquitous computing and mobile sensing to represent human motion characteristics from continuous accelerometer data streams~\cite{bhattacharya14using,hammerla13preserving,plotz11feature}. However, the method has attracted very little attention outside the sensing domain. The simplicity and fast computation time of the ECDF features make it a viable option for using it in static web page analysis. Contrary to mobile sensing, in this paper we primarily focus on discrete reputation ratings and explore the representation power of ECDF features to obtain clues about the content safety of web pages. Figure~\ref{fig:ecdfOverview} shows a pictorial overview of the basic idea of extracting ECDF-based features from a set of embedded web links. 

More formally, let $R = \{r_1, r_2, \ldots, r_n\}$ denotes the set of available reputation ratings of all the embedded web links, where $r_i \in \mathbb{I}_{[0, 100]},\, \forall i \in \{1,\ldots,n\}$. The ECDF $\mathcal{P}_c(r)$ of $R$ can be computed as below:
\begin{eqnarray}
\mathcal{P}_c(r) = p(X \le r),\label{eqn:ecdf}
\end{eqnarray}
where, $p(r)$ is the probability of observing an embedded web link with a reputation rating of $r$ and $X$ is a random variable that takes values from $R$. For example, Figure~\ref{fig:histRS} shows an exemplary histogram of reputation ratings of web links found within a web page and Figure~\ref{fig:ecdfExample} shows the corresponding ECDF computed using Equation~\ref{eqn:ecdf}. Note that $\mathcal{P}_c(r)$ is defined on the entire range of the reputation ratings for embedded web links and is a monotonically increasing function. 

Often the distribution of reputation ratings for embedded links is multi-modal, e.g., as in our example shown in Figure~\ref{fig:histRS}. In order to learn from such distributions, a recognition system should extract descriptors that relate to the shape and spatial position of the modes~\cite{hammerla13preserving}. The shape of the distribution is captured as $\mathcal{P}_c$ increases from $0$ to $1$ (see Figure~\ref{fig:ecdfExample}). To extract a feature vector $\bm{f} \in \mathbb{R}^n$ from the distribution, we first divide the range of $\mathcal{P}_c$, i.e., $[0,1]$, in $n$ equally sized bins with centers respectively at $[b_1,b_2,\ldots,b_n]$. The $i^{th}$ feature component $f_i \in \mathbb{R}$ is then computed as:
\begin{eqnarray}
f_i = \mathcal{P}_c^{-1}(b_i)
\end{eqnarray}
Thus the feature vector $\bm{f}$ captures accurately the shape and positions from the underlying probability function $p(r)$, while the ECDF $\mathcal{P}_c$ can be computed efficiently using Kaplan-Meier estimator~\cite{cox84analysis}.  For completeness, Figure~\ref{fig:ecdfFeatures} shows the extracted ECDF-based feature vector  for $n=75$. The only parameter for the ECDF-based feature extraction method is the number of bins $n$, which controls the granularity with which the shape of the underlying distribution is captured.  


\noindent {\it Adversarial Implications:} ECDF-based features provide an unique opportunity to get important clues about a unknown web page, based on the user ratings of the web pages it refers to. We hypothesize that often a web page that links to other pages with poor ratings, is most likely going to be poor itself and we validate this hypothesis by conducting extensive set of experiments. However, one problem of relying on all outgoing links is that the approach is vulnerable to attacks in which a bad website tries to hide by embedding a large number of web links to good quality web pages. To defend against such an attack one simple idea is to only consider web links with poor ratings while computing the ECDF-based feature set. More specifically, while constructing the set $R$ (see above), we  only allow ratings $r \le C_r$, where $C_r$ is the {\em critical rating threshold} that helps to remove artificial inflation of the set $R$ with good reputation ratings. The choice of $C_r$ can be application dependent and ideally should be adapted based on the overall costs of making false negative predictions. 
%In our evaluation section we will study the influence of $C_r$ on prediction performance in detail.

\subsubsection{Topic Model-based Features}
\label{sssec:topic}

To gain further insights into the type of contents presented on the web pages, we analyze the text in a page and extract a set of features that captures a distribution over a set of topics. In order to learn the topics in an unsupervised manner, we use the {\em Latent Dirichlet Allocation} (LDA) model. The main objective of LDA, or in general in any topic modeling algorithms, is to extract short descriptions of documents, while preserving statistical relationships that are useful, e.g., for document summarization and classification~\cite{blei03latent}. 

\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{pics/LDA}
\caption{Graphical model representing the LDA model used to analyze text form web pages. The boxes represent replications, the shaded circle is the observed variable (word) and unshaded circles are unobserved variables.}
\label{fig:LDA}
\end{figure}

A graphical representation of the model that we use in our analysis of web page texts is shown in Figure~\ref{fig:LDA}. 
%LDA follows a probabilistic generative modeling approach, where documents, in our case web pages containing text, are represented as a mixture of $k$ latent (unobserved) topics, where each topic is characterized by a distribution over a fixed set of words or vocabulary $V$. 
LDA follows a probabilistic generative modeling approach using the {\em bag-of-words} assumption, i.e., the order of occurrence of words within a document is ignored. Under the LDA model, each web page or document $d \in D$  is represented as a mixture of $k$ latent (unobserved) topics denoted by the multinomial variable $\theta_d$ (topic proportion of $d^{th}$ document), where each topic $\beta_k$ is a distribution over the set of words or vocabularies $V$ and is sampled from a Dirichlet distribution with parameter $\eta$. $\theta_d$ is also drawn from a Dirichlet distribution with parameter $\alpha$. $z_{n,d}$ denotes the topic-assignment for the observed word $w_{n,d}$, which is sampled from $\theta_d$. Each word $w_{n,d}$ depends on the topic-assignment variable $z_{n,d}$ and all the topic distributions $\{\beta_k\}_{k=1}^K.$ The joint probability distribution can be given as~\cite{blei12probabilistic}:
\begin{eqnarray}
p(\beta_{1:K}, \theta_{1:D}, z_{1:D}, w_{1:D}) & =  \nonumber \\ 
\prod_{k=1}^K p(\beta_k | \eta) \prod_{d=1}^D p(\theta_d | \alpha) \nonumber \\
\left(  \prod_{n=1}^N p(z_{n,d} | \theta_d) p(w_{n,d} | z_{n,d}, \beta_{1:K})\right) &
\end{eqnarray}

The main task of the topic model is thus to infer the parameters $\beta_k, \theta_d$ and $z_{n,d}$ from the corpus of text, i.e., $w_{1:D}$. The posterior distribution can be written as:
\begin{eqnarray}
p(\beta_{1:K}, \theta_{1:D}, z_{1:D} |  w_{1:D}) = \frac{p(\beta_{1:K}, \theta_{1:D}, z_{1:D}, w_{1:D})}{p(w_{1:D})} \label{eqn:topic}
\end{eqnarray}
Although there are variational algorithms proposed in the literature for estimating the posterior distribution given in Equation~\ref{eqn:topic}, we use a Gibbs sampling-based approach to efficiently approximate it. Once the model parameters are estimated, for a given web page or document $d$ containing the set of words\footnote{As a common pre-processing step, we remove all frequently occurring words (in the language) from a document. The process is also carried out during the model training phase.} $w$, we use $p(\theta_d | w, \beta_{1:K})$, i.e., the estimated topic proportion as the feature set for capturing the thematic content of the document.


\noindent {\em Adversarial Implications:} Similarly to the ECDF-based features, the topic model-based features are susceptible to adversarial attacks. As the topic proportion term $p(\theta_d | w, \beta_{1:K})$ captures the relative weight of various topics being described within the text $w$, an attacker can simply add random words that can boost the probability of certain topics. In Section~\ref{sec:discussion} we propose a possible solution to prevent this attack.



\subsection{Classifier Training}
\label{ssec:classifier}

In our recognition framework we opportunistically extract HTML-based ($\bm{f}_h$), JavaScript-based ($\bm{f}_{j}$), ECDF-based ($\bm{f}_e$), and TopicModel-based ($\bm{f}_t$) features to capture salient properties of web pages. We construct a labeled dataset as follows:
\begin{eqnarray}
W_c & = & \{(\bm{F}^1, y^1), (\bm{F}^2, y^2), \ldots, (\bm{F}^n, y^n)\}, \\
\mbox{where,  } \bm{F}^i & = & (\bm{f}^i_h, \bm{f}^i_j, \bm{f}^i_e, \bm{f}^i_t,) \nonumber
\end{eqnarray}
One challenge of an opportunistic feature extraction procedure is often one or more types of features are not available. For example, in our web page safety prediction task, not all web pages use JavaScript, contain embedded links, or use textual descriptions. However, we assume that the HTML-based features are always available for a web page. A classification technique thus has to overcome the problem of feature unavailability. Existing approaches such as~\cite{canali11prophiler, Ma09BeyondBlacklists, seifert08identification, seifert08identify}, have limited generalizability under this learning setting. To overcome the problem, we first train four classifiers $\mathcal{C}_h$, $\mathcal{C}_j$, $\mathcal{C}_e$, and $\mathcal{C}_t$ using HTML, JavaScript, ECDF, and Topic model-based features respectively and combine them following a maximum a posterior (MAP) approach to generate the final recognizer. Figure~\ref{fig:classification} provides a pictorial overview of our hierarchical classification approach. 

\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{pics/classificationOverview}
\caption{Our proposed classification framework follows a hierarchical approach and combines the posterior probabilities obtained from individual feature sets to compute the maximum a posterior probability to infer the final category of a web page.}
\label{fig:classification}
\end{figure}

More specifically, in case of our web page safety detection problem, the main objective is to predict the safety or class of a web page given its features $(\bm{f}_h, \bm{f}_j, \bm{f}_e, \bm{f}_t)$. Note that one or more of $(\bm{f}_j, \bm{f}_e, \bm{f}_t)$ can be missing. Given the classifier $\mathcal{C}_h$, we compute the posterior probabilities for all the target classes, i.e., we compute:
\begin{eqnarray}
p_h(c_i | \bm{f}_h), \forall i \in \{1,\ldots, C\},
\end{eqnarray}
where $C$ is the total number of classes present. Similarly, we compute the posterior probabilities $p_j(\cdot), p_e(\cdot)$ and $p_t(\cdot)$ using the other three classifiers. Note that, if a feature type is missing, then the corresponding posterior probabilities are all zero. The posterior probabilities can be combined to generate the overall belief as follows:
\begin{eqnarray} 
p^*(c_i | \bm{f}_h, \bm{f}_j, \bm{f}_e, \bm{f}_t) & = &\nonumber \\ 
w_h \cdot p_h(c_i | \bm{f}_h)  &+&  w_j \cdot p_h(c_i | \bm{f}_j)  \,\,\,\,+ \nonumber \\
w_e \cdot p_h(c_i | \bm{f}_e) &+&  w_h \cdot p_t(c_i | \bm{f}_t), \label{eqn:combined}
\end{eqnarray}
where, $w_h, w_j, w_e$ and $w_t$ are respectively the weighs for the individual classifiers used to influence the final belief. In our experiments the weights are selected such that $w_h + w_j + w_e + w_t = 1$. One straight forward solution is to assign equal weighs for the classifier in Equation~\ref{eqn:combined}. However, a better approach is to adapt the weights of individual classifiers based on their prediction confidence. In this work we follow an adaptive weight selection method for the classifiers based on the difficulty level of the classification task at hand. More specifically, given a feature set $\bm{f}$ and the corresponding class labels $y$, we compute the Fukunaga class separability score~\cite{fukunaga90introduction}. The Fukunaga score relies on computing both the {\em within-class} and {\em between-class} scatter matrices. Let $n_i$ be the number of samples of the feature set belonging to class $c_i$ of $C$ different classes. Further, let $\bm{\mu}_i$ and $\bm{\mu}$ respectively be the mean for class $c_i$ and the global mean. The within-class and between-class scatter matrices $S_W$ and $S_B$ can be computed as follows:
\begin{eqnarray}
S_W &=& \sum_{i=1}^C \left[ \sum_{j=1}^{n_i} (\bm{f}_{i,j} - \bm{\mu}_i) (\bm{f}_{i,j} - \bm{\mu}_i)^T\right]\\
S_B &=& \sum_{i=1}^C n_i (\bm{\mu}_i - \bm{\mu}) (\bm{\mu}_i - \bm{\mu})^T
\end{eqnarray}
Then the Fukunaga score is computed as:
\begin{eqnarray} 
Separability = Tr(S_B / S_W)
\end{eqnarray}
For each classifier we compute the separability score and normalize them. The normalized score is then used as the respective weight for a classifier. The final predicted class $\hat{y}$ is then computed as:
\begin{eqnarray} 
\hat{y} = arg \max_{i} \,\,p^*(c_i |  \bm{f}_h, \bm{f}_j, \bm{f}_e, \bm{f}_t)
\end{eqnarray}




\subsection{Datasets}
\label{sssec:datasets}

%To evaluate the performances of our proposed novel feature extraction
%techniques and the hierarchical classification methodology, in this
%section we describe in detail the dataset used in our experiments and
%the evaluation metric used for comparisons.

To perform an extensive and systematic study, we generated a pool of over $140,000$ URLs. Within this pool, $80,000$ URLs are selected from the WOT database corresponding to web pages with positive reputation ratings. The rest of the $60,000$ URLs represents webpages with negative ratings. 
%These URLs are selected from Google Analytics API provided by the WOT. 

Once the URL pool is generated, we crawled the web pages selected from the pool to extract HTML, JavaScript, ECDF and topic model-based features. We also query the WOT API to obtain the reputation ratings for every page. In Table~\ref{tbl:dataset}, we highlight summary statistics of our dataset. More specifically, we show how many URLs (dataset size) contain valid features. For example, the row with `Feature set' HTML + JavaScript indicates that the number of URLs, where HTML and JavaScript-based features are both available. The results given in Table~\ref{tbl:dataset} highlight the fact that seldom all features types can be extracted from web pages and the proportions can be highly imbalanced. For example, for automatically learning the topics we primarily focus on english texts and use automatic translation services through available APIs for a small number of non-english languages, which results in around $28\%$ of all the URLs having all feature types available.


\begin{table}[!t]
\centering
\begin{tabular} {|c|c|c|}
\hline
{\bf Links} & {\bf Feature set}         &   {\bf Reputation}\\  
\hline
$89,220$ 	&  WOT + HTML  & Trust\\
\hline
$77,168$ 	&  WOT + HTML +  JavaScript & Trust\\
\hline
%\multirow{2}{*}{$72,366$} & WOT rating  + HTML + JavaScript & \multirow{2}{*}{Trustworthiness}\\
%				    &	+ ECDF	&	\\
%\multirow{2}{*}{$35,159$} & WOT rating  + HTML + JavaScript & \multirow{2}{*}{Trustworthiness}\\
%				    &	+ ECDF + Topic	&	\\
%\hline				    
\multirow{2}{*}{$46,785$} & WOT  + HTML +  JavaScript & \multirow{2}{*}{Trust}\\
				    &	+ ECDF	&	\\				    				    
\hline				    
\multirow{2}{*}{$43,675$} & WOT  + HTML + JavaScript & \multirow{2}{*}{Trust}\\
				    &	+ ECDF + Topic	&	\\				    				    				    
\hline
\hline
$84,714$ 	&  WOT + HTML  & Child safety\\
\hline
$73,566$ 	&  WOT + HTML +  JavaScript & Child safety\\
\hline
%\multirow{2}{*}{$69,268$} & WOT rating  + HTML + JavaScript & \multirow{2}{*}{Child safety}\\
%				    &	+ ECDF	&	\\
%\multirow{2}{*}{$34,593$} & WOT rating  + HTML + JavaScript & \multirow{2}{*}{Child safety}\\
%				    &	+ ECDF + Topic	&	\\
%\hline				    
\multirow{2}{*}{$45,161$} & WOT  + HTML +  JavaScript & \multirow{2}{*}{Child safety}\\
				    &	+ ECDF	&	\\				    				    
\hline				    
\multirow{2}{*}{$42,334$} & WOT  + HTML + JavaScript & \multirow{2}{*}{Child safety}\\
				    &	+ ECDF + Topic	&	\\	
\hline
\end{tabular}
\caption{Summary of the dataset used in our experiments, indicating availability of various WOT ratings and features in two reputation dimensions.}
\label{tbl:dataset}
\end{table}


% \subsubsection{Data Pre-processing}
% Given a URL, the WOT system returns a set of reputation scores $(r_t, r_c)$, where $r_t$ is the crowdsourced rating for trustworthiness,  and $r_c$ is the rating for child safety. Moreover, the returned reputation scores $r_t,r_c \in \mathbb{R}_{[0, 100]}$. While performing predictions, one solution is to directly use the reputation scores and train a regression model. However, as far as user's safety is concerned, often a binary indicator is more suitable, e.g., indicating whether a web is trustworthy or safe for a child. Accordingly, in this paper we formulate the web safety detection task as a classification problem. 

% Before training a classifier, we convert the reputation scores obtained for all the URLs into two class based on the reference levels used by the WOT. For example, out of five category levels as used by WOT (see Figure~\ref{fig:wot_score}), we combine the lowest three categories as the poor/bad category and consider the top two categories as the good category. In other words, this segregation translates to consider a web page as bad if its reputation score is less than $60$, otherwise the web page is considered good. Hence, we formulate the web safety detection problem as a binary classification task. Note that, the feature representation and the hierarchical classification techniques proposed in this paper are generic and directly applicable in other classification settings, where the number of target classes are more than two.


%\todo{JL's Text Start} To derive our detection models, we constructed two datasets, which contain links with ratings in trustworthiness (TR) and child-safety (CS) respectively. The links were gathered from WOT database and  dataset as of January 1st, 2014. The ratings were obtained from the WOT API, and labelled as one of with Excellent (E), good (G), unsatisfactory (U), poor (P) and very poor (VP) along each of the two dimensions (TR and CS).  The CS data set is a little smaller than TR dataset, because there are some links have no ratings in child-safety. The datasets are summarized in Table~\ref{dataset} \todo{END}.



%\subsubsection{All-features-available}
%\subsubsection{Opportunistic}

%\begin{table}[!t]
%\caption{The dataset used for our experiments.}
%\centering
%\begin{tabular} {| c | c | c |c|c|c|c|}
%\hline
%  \textbf{Dataset name}         &    \textbf{E}      &    \textbf{G}  &  \textbf{U}  &   \textbf{P}   &  \textbf{VP}   &   \textbf{Total}  \\  \hline
%   \textbf{TR}      & 5,452 & 2,449 & 2,889 & 2,394 & 3,281 & 16,465    \\  \hline
%   \textbf{CS}            & 7,481 & 1,997 & 895  & 935 & 5,082 & 16,390 \\ 
%\hline
%\end{tabular}
% \label{dataset}
%\end{table}

\subsection{Results}
\label{sec:experiments}

\input{chapters/results.tex}


In this section we report results from an extensive set of experiments to systematically study the influence of individual feature types and their various combinations on the overall prediction performance. In the first set of experiment, we apply our proposed classification technique on datasets where all of HTML, JavaScript, ECDF (computed based on bad links only), and Topic model-based features are available. In case of reputation dimension of trustworthiness and child safety, considering all feature availability results in $24,947$ and $25,202$ URLs respectively.

%The main reason for this subset selection is to keep the training and the test sets (comprising of identical URLs) fixed during different folds of the classification experiments. Fixed training and test sets helps us to perform statistical testing to verify if the performance improvement is significant. Additionally, to match the practical scenario, we also perform experiments on the entire dataset, where we opportunistically take into account availability of different types of features. While performing the opportunistic experiments we only consider those URLs that have at least valid HTML features. In case of trustworthiness, this generates a dataset comprising of $89,220$ URLs and $84,714$ URLs in case of child safety. 

%For the purpose of drawing comparative analysis of different classification performances under different feature types, we primarily focus on two dataset types. In the first type, we consider a subset of our dataset, where all feature types are available. 



Once the experimental dataset is selected, we run a set of classification experiments using five fold cross validations, while using the same training and test data folds in all the experiments. This allows us to draw direct comparisons among all experiments. Moreover, while generating the cross validation dataset we perform stratified sampling technique to maintain similar class distribution within the training and test folds. We begin our experiments by considering a single type of features, then perform experiments considering all possible combinations of two feature types, followed by all combinations of three features, and lastly we report classification performance using all four feature types. Table~\ref{tbl:4featuresBadLink} summarizes all $15$ possible experimental scenarios for both the reputation dimensions. Note that, before running the cross validation experiments, we perform feature selection (see Section~\ref{ssec:profRes} for details) of all the feature types except ECDF, as the performance of ECDF features depends on capturing the overall shape and position of modes of the underlying distribution. If more than one feature types are used, then we determine the relative strength of a classifier by computing the Fukunaga class separability score (see Section~\ref{ssec:classifier}). For all the classification experiments we use C4.5 decision tree as the basic classifier.

Our experimental results indicate that when individual feature types are considered, the overall classification performances ($F_1$-score\footnote{To overcome the effect of class imbalances in test dataset, as the primary evaluation metric we report the expected $F_1$-score. The expectation is computed by performing weighted averaging of the class specific $F_1$-scores, where class proportions are used as the weights.}) of HTML, JavaScript, ECDF, and Topic model based features are respectively $71.2\%$, $70.5\%$, $72.4\%$, and $72.7\%$ in case of trustworthiness. McNemar chi-squared test shows that both the content-related features (ECDF and Topic) perform significantly better ($p < 0.05$) than the structural (HTML, JavaScript) features. In general, considering two types of features improves the prediction performance as compared to single feature type, both in terms of $F_1$-score and false negatives. It is observed that the ECDF features, when combined with a structural feature type, achieves a better $F_1$-score of $76.3\%$. The improvement of classification performance continues when three types of features are combined together. The best $F_1$-score is achieved when all the features are combined together. A very similar trend is also observed for the reputation dimension child safety. E.g., the best performance, $F_1$-score = $86\%$, is observed when all four feature types are combined together. In general, the recognition system performs well in case of predicting child safety. Interestingly, the performance of the HTML + JavaScript features in the experiments closely follow the Prophiler\footnote{The difference between Prophiler and the HTML+Javascript feature-set analyzed here is only in how the results of the individual classifiers are combined. Prophiler uses OR, while we use a adaptive hierarchical classification approach.}.

\begin{table*}[!t]
\centering
\caption{$F_1$-score comparisons among various feature set combinations.}
\begin{tabular} {|c|c|c|c|}
\hline
{\bf Featureset / $F_1$-scores (Trust, Child)}         &   {\bf Featureset / $F_1$-scores (Trust, Child)} & {\bf Trustworthiness}      &   {\bf Child safety}\\
				&				& {\bf (p value)}		& {\bf (p value)}\\
\hline
HTML ($71.2, 80.9$)	& ECDF ($72.4, 80.8$)   & $< 0.05$ & - \\
\hline
HTML ($71.2, 80.9$)	& Topic ($72.7, 83.8$)  & $< 0.01$ & $< 0.01$\\
\hline
ECDF ($72.4, 80.8$)	& Topic ($72.7, 83.8$) & - & $< 0.01$\\
\hline
HTML + JavaScript ($73.6, 82.3$) 	& ECDF + Topic ($75.2, 85.1$) & $< 0.01$ & $< 0.01$\\
\hline
HTML + JavaScript ($73.6, 82.3$) 	& HTML + JavaScript + ECDF ($76.7, 84.1$)  & $< 0.01$ & $< 0.01$\\
\hline
HTML + JavaScript ($73.6, 82.3$) 	& HTML + JavaScript + Topic ($75.8, 85.3$)  & $< 0.01$ & $< 0.01$\\
\hline
HTML + JavaScript + ECDF ($76.7, 84.1$)	& HTML + JavaScript + ECDF + Topic ($77.8, 86.0$)  & $< 0.05$ & $< 0.01$\\
\hline
HTML + JavaScript + Topic ($75.8, 85.3$)	& HTML + JavaScript + ECDF + Topic ($77.8, 86.0$) & $< 0.01$ & $< 0.01$\\
\hline
\end{tabular}
\label{tbl:statTest}
\end{table*}



\begin{table*}[!t]
\centering
\caption{$F_1$-score comparisons among various feature set combinations for the Opportunistic classification experiments.}
\begin{tabular} {|c|c|c|c|}
\hline
{\bf Featureset  / $F_1$-scores (Trust, Child)}         &   {\bf Featureset  / $F_1$-scores (Trust, Child)} & {\bf Trustworthiness}      &   {\bf Child safety}\\
				&				& {\bf (p value)}		& {\bf (p value)}\\
\hline
HTML + JavaScript ($69.6, 71.6$) 	& HTML + ECDF ($72.4, 73.5$) & $< 0.01$ & $< 0.01$\\
\hline
HTML + JavaScript ($69.6, 71.6$)	& HTML + ECDF + Topic ($73.9, 75.9$)  & $< 0.01$ & $< 0.01$\\
\hline
HTML + JavaScript ($69.6, 71.6$)	& HTML + JavaScript + ECDF ($74.3, 75.0$)  & $< 0.01$ & $< 0.01$\\
\hline
HTML + JavaScript ($69.6, 71.6$)	& HTML + JavaScript + Topic ($73.4, 76.2$) & $< 0.01$ & $< 0.01$\\
\hline
HTML + JavaScript + ECDF ($74.3, 75.0$) & HTML + JavaScript + ECDF + Topic ($75.3, 77.3$) & $< 0.01$ & $< 0.01$\\
\hline
HTML + JavaScript + Topic ($73.4, 76.2$)  & HTML + JavaScript + ECDF + Topic ($75.3, 77.3$) & $< 0.01$ & $< 0.01$\\
\hline
\end{tabular}
\label{tbl:statTestOpportunistic}
\end{table*}


In order to systematically compare the performances reported in Table~\ref{tbl:4featuresBadLink}, in Table~\ref{tbl:statTest} we summarize statistical significance testing, using McNemar Chi-squared test, for some salient pairs of feature sets. The p-values $< 0.05$ and $<0.01$  respectively denotes a confidence level of $95\%$ and $99\%$. From the table it can be seen that the content-based features perform significantly better (higher $F_1$-score) than the structural features for both reputation dimensions. In case of child safety, topic model-based feature set works significantly better than the ECDF-based features, whereas no difference is observed between these pair of features in case of trustworthiness. For both the dimensions, combining all the features improved the recognition performance significantly.


Contrary to the experimental framework explained in the above experiments, in real world situations often one or more feature dimensions are missing. To evaluate our proposed classification approach under  naturalistic setting, as the last set of classification experiments, we run experiments using our entire URL dataset. As mentioned before, we assume that at least HTML features are always available. Following the same procedure as before, we run a five fold cross validation experiments for all possible feature type combinations. The classification performances are given in Table~\ref{tbl:opportunistic}. For both reputation dimensions, the best performance is exhibited when all four feature types are combined together. Recall from Section~\ref{ssec:classifier} (Figure~\ref{fig:classification}) that if a feature type is missing from a web page then the classifier trained on the feature type returns all zero posterior probabilities, thus has no contribution to the safety prediction of the web page. The opportunistic addition of available features, in general, decreases the overall false negative predictions. 

For completeness of our analysis, we summarize salient statistical significance tests for the experiments in Table~\ref{tbl:statTestOpportunistic}. The results indicate that the ECDF features (considering only bad links) combined with HTML features improves the prediction performance significantly over HTML and JavaScript features (similar to Prophiler). The opportunistic combination of all feature types results in statistically significant performance over all other possible feature type combinations on our entire dataset with close to $90,000$ web pages.





==> performance.tex <==
%!TEX root = ../submission.tex

\section{Performance Considerations}
\label{sec:performance}

In this section we summarize the performance of our various feature extraction techniques and report the average running time needed for computing them. For the purpose of computing the average extraction time we have randomly selected $1,000$ URLs from our dataset (see Section~\ref{sssec:datasets}) and carefully logged the time required to extract HTML + JavaScript, ECDF, and Topic model-based features on a standard Linux desktop computer (8 Gb RAM, 2.4 GHz processor). In case of Topic model features we also noted down the  time cost for performing translation of non-english web pages using an API. Table~\ref{tbl:timePerformance} summarizes the time analysis of our feature extraction methods. On average $3.1 \,\,s$ is needed per web page to extract the structural features, whereas only $1.9 \,\,s$ per web page is needed for obtaining the ECDF features. The topic model feature computation requires the least amount of average time per web page ($1.3 \,\,s$), when no translation is required. However, for non English web pages the average feature computation time increases to $3.4 \,\,s$ per page. The feature set collection time needed in our approach, especially for the content features (without translation), is smaller than the reported time of $3.06 \,\, s$ by Prophiler. Thus, our proposed feature extraction procedure is highly suitable for real time safety prediction of web pages.


\begin{table}[!t]
\centering
\caption{Time Analysis for Fetching Various Features.}
\begin{tabular} {|c|c|}
\hline
{\bf Feature type} & {\bf Average fetch time}\\  
\hline
HTML + JavaScript & 3.1 s / link\\
ECDF & 1.9 s / link\\
Topic + translation & 3.4 s / link\\
Topic + without translation & 1.3 s / link\\
\hline
\end{tabular}
\label{tbl:timePerformance}
\end{table}


==> results.tex <==
%!TEX root = ../submission.tex

%\begin{table*}[!p]
%\centering
%\caption{Predictive Performance using 5-fold cross validations while considering only bad embedded links for the ECDF features. The selected dataset has valid measurements for all the feature dimensions. Basic Classifier = Decision Tree.}
%\begin{tabular} {|c|c|c|c|c|c|c|}
%\hline
%{\bf Dataset size} & {\bf Featureset}         &   {\bf Reputation}      &   {\bf Precision}  &  {\bf Recall}  & {\bf $F_1$-score} & {\bf False negatives}\\  
%\hline
%$46,785$ 	& HTML 	& Trust	&   $69.8$ 	& $69.8$  	&  $69.8$	&$14.6\%$\\
%$46,785$ 	& JavaScript 	& Trust	&   $68.6$ 	& $68.6$  	&  $68.5$	& $14.4\%$\\
%$46,785$ 	& ECDF 	& Trust	&   $71.1$ 	& $71.1$  	&  $71.1$	& $15.0\%$\\
%\hline
%$46,785$ 	& HTML + JavaScript 	& Trust	&   $72.1$ 	& $72.1$  	&  $72.1$	& $13.4\%$\\
%$46,785$ 	& JavaScript + ECDF 	& Trust	&   $73.9$ 	& $73.8$  	&  $73.8$	& $13.7\%$\\
%$46,785$ 	& HTML + ECDF 	& Trust	&   $76.8$ 	& $76.8$  	&  $76.8$	& $11.7\%$\\
%\hline
%$46,785$ 	& HTML + JavaScript + ECDF 	& Trust	&  ${\bf 77.7}$ 	& ${\bf 77.7}$  	&  ${\bf 77.7}$ & ${\bf 10.8\%}$\\
%\hline
%\hline
%$45,161$ 	& HTML 	& Child-safety	&   $73.3$ 	& $73.5$  	&  $73.4$	& $12.6\%$\\
%$45,161$ 	& JavaScript 	& Child-safety	&   $72.9$ 	& $73.0$  	&  $72.9$	& $12.7\%$\\
%$45,161$ 	& ECDF 	& Child-safety	&   $73.2$ 	& $73.3$  	&  $73.2$	& $13.1\%$\\
%\hline
%$45,161$ 	& HTML + JavaScript 	& Child-safety	&   $75.9$ 	& $76.1$  	&  $76.0$	& $10.7\%$\\
%$45,161$ 	& JavaScript + ECDF 	& Child-safety	&  $76.5$ 	& $76.7$  	&  $76.6$	& $10.8\%$\\
%$45,161$ 	& HTML + ECDF 	& Child-safety	&   $78.3$ 	& $78.4$  	&  $78.3$	& $9.7\%$\\
%\hline
%$45,161$ 	& HTML + JavaScript + ECDF 	& Child-safety	&   ${\bf 79.9}$ 	& ${\bf 80.0}$  	&  ${\bf 79.9}$	& ${\bf 8.4\%}$\\
%\hline
%\end{tabular}
%\label{tbl:3featuresBadLinkOnly}
%\end{table*}

\begin{table*}[!t]
\centering
\caption{Predictive Performance using 10-fold cross validations while considering only bad embedded links for the ECDF features. The selected dataset has valid measurements for all the feature dimensions. Basic Classifier = Random Forest.}

\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\bf No. of URLs} & \multirow{2}{*}{\bf Reputation} & \multicolumn{4}{c|}{\bf Feature sets}      &    \multirow{2}{*}{\bf Precision (\%)}  &   \multirow{2}{*}{\bf Recall (\%)}  &  \multirow{2}{*}{\bf F-Score (\%)} & \multirow{2}{*}{\bf FNR (\%)} & \multirow{2}{*}{\bf FPR (\%)}\\  
\cline{3-6}
& & {\bf HTML} & {\bf JavaScript} & {\bf ECDF} & {\bf Topic} & & & & &\\
\hline
\multirow{15}{*}{\bf 43,675} & \multirow{15}{*}{\bf Trustworthiness} & \checkmark &  &  &   & $75.8$ & $75.7$ & $75.7$ & $23.6$ & $24.9$\\
&  &  & \checkmark &  &  & $74.9$ & $74.9$ & $74.9$ & $25.1$ & $25.1$\\
&  &  & & \checkmark &  & $70.5$ & $70.5$ & $70.5$ & $29.0$ & $29.9$\\
&  &  &  & & \checkmark & $74.9$ &$74.9$ & $74.9$ & $24.5$ & $25.7$\\
\cline{3-11}
& & \checkmark & \checkmark &  &  & $76.8$ & $76.8$ & $76.8$ & $22.6$ & $23.8$\\
& & \checkmark &  & \checkmark &  & $77.3$ & $77.3$ & $77.3$ & $23.9$ & $21.6$\\
& & \checkmark &  &  & \checkmark & $78.7$ & $78.7$  & $78.7$ & $20.2$ & $22.4$\\
& &  & \checkmark & \checkmark &  & $74.1$ & $74.1$ & $74.1$ & $26.3$ & $25.5$\\
& &  & \checkmark &  & \checkmark & $77.7$ & $77.7$ & $77.7$ & $21.7$ & $22.8$\\
& &  &  & \checkmark & \checkmark & $79.2$ & $79.2$ & $79.2$ & $21.0$ & $20.5$\\
\cline{3-11}
& & \checkmark & \checkmark &  \checkmark &  & $79.3$ & $79.3$ & $79.3$ & $21.7$ & $19.8$\\
& & \checkmark &  \checkmark &  & \checkmark & $79.6$ & $79.6$ & $79.6$ & $19.6$ & $21.3$\\
& & \checkmark &  & \checkmark & \checkmark & $81.6$ & $81.6$ & $81.6$ & $17.9$ & $18.8$\\
& &  &  \checkmark & \checkmark & \checkmark & $81.0$ & $81.0$ & $81.0$ & $19.0$ & $19.1$\\
\cline{3-11}
& & \checkmark & \checkmark & \checkmark & \checkmark & \bm{$82.4$} & \bm{$82.4$} & \bm{$82.4$} & \bm{$17.3$} & \bm{$18.0$}\\
\hline
\hline
\multirow{15}{*}{\bf 42,334} & \multirow{15}{*}{\bf Child safety} & \checkmark &  &  &   & $79.2$ & $79.2$ & $79.2$ & $16.7$ & $26.4$\\
&  &  & \checkmark &  &  & $78.6$ & $78.7$ & $78.7$ & $16.5$ & $27.9$\\
&  &  & & \checkmark &  & $73.4$ & $73.4$ & $73.4$ & $22.4$ & $32.4$\\
&  &  &  & & \checkmark & $81.0$ &$80.9$ & $80.9$ & $17.9$ & $20.8$\\
\cline{3-11}
& & \checkmark & \checkmark &  &  & $79.9$ & $80.0$ & $79.9$ & $15.8$ & $26.0$\\
& & \checkmark &  & \checkmark &  & $79.2$ & $79.3$ & $79.2$ & $17.2$ & $25.6$\\
& & \checkmark &  &  & \checkmark & $83.2$ & $83.2$  & $83.2$ & $14.7$ & $19.7$\\
& &  & \checkmark & \checkmark &  & $76.8$ & $76.8$ & $76.8$ & $19.4$ & $28.4$\\
& &  & \checkmark &  & \checkmark & $82.7$ & $82.7$ & $82.7$ & $15.7$ & $19.6$\\
& &  &  & \checkmark & \checkmark & $83.2$ & $83.1$ & $83.1$ & $15.8$ & $18.6$\\
\cline{3-11}
& & \checkmark & \checkmark &  \checkmark &  & $81.5$ & $81.6$ & $81.5$ & $14.7$ & $23.6$\\
& & \checkmark &  \checkmark &  & \checkmark & $83.9$ & $84.0$ & $84.0$ & $13.4$ & $19.6$\\
& & \checkmark &  & \checkmark & \checkmark & $84.9$ & $84.8$ & $84.8$ & $13.5$ & $17.5$\\
& &  &  \checkmark & \checkmark & \checkmark & $84.3$ & $84.3$ & $84.3$ & $14.3$ & $17.7$\\
\cline{3-11}
& & \checkmark & \checkmark & \checkmark & \checkmark & \bm{$85.3$} & \bm{$85.3$} & \bm{$85.3$} & \bm{$12.8$} & \bm{$17.3$}\\
\hline
\end{tabular}
\label{tbl:4featuresBadLink}
\end{table*}



%\begin{table*}[!t]
%\centering
%\caption{Predictive Performance using 5-fold cross validations while considering only bad embedded links for the ECDF features. The selected dataset has valid measurements for all the feature dimensions. Basic Classifier = Random Forest.}
%
%\begin{tabular} {|c|c|c|c|c|c|c|c|}
%\hline
%\multirow{2}{*}{\bf Links} & \multirow{2}{*}{\bf Featureset}         &   \multirow{2}{*}{\bf Reputation}      &    {\bf Precision}  &   {\bf Recall}  &  {\bf Avg. $F_1$-score} & {\bf FPR} & {\bf FNR}\\  
% &         &      &    {\bf (\%)}  &  {\bf (\%)}  & {\bf (\%)} & {\bf (\%)} & {\bf (\%)} \\  
%\hline
%$43,675$ 	& HTML 	& Trustworthiness	&   $69.4$ 	& $69.4$  	&  $69.4$	& $15.6$  & $15.0$\\
%$43,675$ 	& \cellcolor{Gray}JavaScript 	& Trust	&  $68.7$ 	& $68.7$  	&  $68.7$	&$16.8$ & $14.5$\\
%$43,675$ 	& ECDF 	& Trust	&   $70.7$ 	& $70.7$  	&  $70.7$	& $14.1$ & $15.2$\\
%$43,675$ 	& Topic 	& Trust	&   $67.0$ 	& $67.0$  	&  $67.0$	& $16.9$ & $16.2$\\
%\hline
%$43,675$ 	& HTML + JavaScript 	& Trust	&   $71.6$ & $71.6$  &  $71.6$	& $14.7$ & $13.7$\\
%$43,675$ 	& HTML + ECDF 	& Trust	&   $76.2$ 	& $76.2$  	&  $76.2$	& $11.5$ & $12.3$\\
%$43,675$ 	& HTML + Topic 	& Trust	&   $69.7$ 	& $69.7$  	&  $69.7$	& $15.4$ & $15.5$\\
%$43,675$ 	& JavaScript + ECDF 	& Trust	&   $73.5$ 	& $73.5$  	&  $73.5$	& $12.6$ & $13.9$\\
%$43,675$ 	& JavaScript + Topic 	& Trust	&   $69.7$ 	& $69.7$  	&  $69.7$	& $15.3$ & $15.0$\\
%$43,675$ 	& ECDF + Topic 	& Trust	&   $70.7$ 	& $70.7$  	&  $70.7$	& $14.8$ & $14.6$\\
%\hline
%$43,675$ 	& HTML + JavaScript + ECDF 	& Trust	&   ${\bf 77.7}$ 	& ${\bf  77.7}$  	&  ${\bf 77.7}$ & ${\bf 11.0}$ & ${\bf 11.3}$\\
%$43,675$ 	& HTML + JavaScript + Topic 	& Trust	&   $71.3$ 	& $71.3$  	&  $71.3$ & $14.5$ & $14.1$\\
%$43,675$ 	& HTML + ECDF + Topic 	& Trust	&   $74.2$ 	& $74.2$  	&  $74.2$ & $13.1$ & $12.7$\\
%$43,675$ 	& JavaScript + ECDF + Topic 	& Trust	&   $73.1$ 	& $73.1$  	&  $73.1$ & $13.6$ & $13.3$\\
%\hline
%$43,675$ 	& HTML + JavaScript + ECDF + Topic 	& Trust	&   $75.7$ 	& $75.6$  	&  $75.6$ & $12.5$ & $11.9$\\
%\hline
%\hline
%$42,334$ 	& HTML 	& Child safety	&   $73.5$ 	& $73.6$  	&  $73.5$	& $13.8$ & $12.6$\\
%$42,334$ 	& JavaScript 	& Child safety	&   $72.7$ 	& $72.8$  	&  $72.7$	&$14.5$ & $12.7$\\
%$42,334$ 	& ECDF 	& Child safety	&   $73.3$ 	& $73.3$  	&  $73.3$	& $13.4$ & $13.3$\\
%$42,334$ 	& Topic 	& Child safety	&   $74.4$ 	& $74.4$  	&  $74.4$	& $12.9$ & $12.6$\\
%\hline
%$42,334$ 	& HTML + JavaScript 	& Child safety	&   $75.9$ 	& $76.0$  	&  $75.9$	& $13.0$ & $11.0$\\
%$42,334$ 	& HTML + ECDF 	& Child safety	&   $78.1$ 	& $78.2$  	&  $78.2$	& $11.6$ & $10.2$\\
%$42,334$ 	& HTML + Topic 	& Child safety	&   $76.5$ 	& $76.5$  	&  $76.5$	& $12.0$ & $11.5$\\
%$42,334$ 	& JavaScript + ECDF 	& Child safety	&   $76.4$ 	& $76.4$  	&  $76.4$	& $12.5$ & $11.0$\\
%$42,334$ 	& JavaScript + Topic 	& Child safety	&   $76.4$ 	& $76.4$  	&  $76.4$	& $12.0$ & $11.5$\\
%$42,334$ 	& ECDF + Topic 	& Child safety	&   $76.4$ 	& $76.4$  	&  $76.4$	& $11.8$ & $11.8$\\
%\hline
%$42,334$ 	& HTML + JavaScript + ECDF 	& Child safety	&   $80.0$ 	& $80.1$  	&  $80.0$ & $11.0$ & $8.9$\\
%$42,334$ 	& HTML + JavaScript + Topic 	& Child safety	&  $76.6$ 	& $76.6$  	&  $76.6$ & $12.0$ & $11.4$\\
%$42,334$ 	& HTML + ECDF + Topic 	& Child safety	&   $77.2$ 	& $77.2$  	&  $77.2$ & $11.5$ & $11.3$\\
%$42,334$ 	& JavaScript + ECDF + Topic 	& Child safety	&   $77.2$ 	& $77.2$  	&  $77.2$ & $11.5$ & $11.3$\\
%\hline
%$42,334$ 	& HTML + JavaScript + ECDF + Topic 	& Child safety	&  $78.1$ 	& $78.1$  	&  $78.1$ & $11.2$ & $10.7$\\
%\hline
%\end{tabular}
%\label{tbl:4featuresBadLink}
%\end{table*}

\begin{table*}[!t]
\centering
\caption{Opportunistic Predictive Performance using 10-fold cross validations while considering only bad embedded links for the ECDF features. Basic Classifier = Random Forest.}

\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\bf No. of URLs} & \multirow{2}{*}{\bf Reputation} & \multicolumn{4}{c|}{\bf Feature sets}      &    \multirow{2}{*}{\bf Precision (\%)}  &   \multirow{2}{*}{\bf Recall (\%)}  &  \multirow{2}{*}{\bf F-Score (\%)} & \multirow{2}{*}{\bf FNR (\%)} & \multirow{2}{*}{\bf FPR (\%)}\\  
\cline{3-6}
& & {\bf HTML} & {\bf JavaScript} & {\bf ECDF} & {\bf Topic} & & & & &\\
\hline
\multirow{8}{*}{\bf 89,220} & \multirow{8}{*}{\bf Trustworthiness} & \checkmark &  &  &   & $73.4$ & $73.9$ & $73.1$ & $45.8$ & $14.3$\\
\cline{3-11}
& & \checkmark & \checkmark &  &  & $74.7$ & $74.9$ & $73.9$ & $47.3$ & $11.7$\\
& & \checkmark &  & \checkmark &  & $75.4$ & $75.1$ & $75.2$ & \bm{$30.4$} & $21.6$\\
& & \checkmark &  &  & \checkmark & $76.5$ & $76.5$  & $75.4$ & $46.2$ & $9.9$\\
\cline{3-11}
& & \checkmark & \checkmark &  \checkmark &  & $77.2$ & $77.2$ & $77.2$ & $31.0$ & $17.9$\\
& & \checkmark &  \checkmark &  & \checkmark & $77.5$ & $77.2$ & $76.0$ & $46.4$ & \bm{$8.6$}\\
& & \checkmark &  & \checkmark & \checkmark & $79.7$ & $79.9$ & $79.6$ & $33.4$ & $12.1$\\
\cline{3-11}
& & \checkmark & \checkmark & \checkmark & \checkmark & \bm{$80.6$} & \bm{$80.7$} & \bm{$80.3$} & $33.9$ & $10.5$\\
\hline
\hline
\multirow{8}{*}{\bf 84,714} & \multirow{8}{*}{\bf Child safety} & \checkmark &  &  &   & $74.9$ & $74.9$ & $74.5$ & $37.5$ & $15.9$\\
\cline{3-11}
& & \checkmark & \checkmark &  &  & $76.5$ & $76.4$ & $75.9$ & $37.0$ & $13.8$\\
& & \checkmark &  & \checkmark &  & $76.0$ & $75.6$ & $75.7$ & $24.4$ & $24.3$\\
& & \checkmark &  &  & \checkmark & $80.7$ & $79.9$  & $79.3$ & $36.3$ & $8.2$\\
\cline{3-11}
& & \checkmark & \checkmark &  \checkmark &  & $77.7$ & $77.6$ & $77.6$ & \bm{$24.5$} & $20.9$\\
& & \checkmark &  \checkmark &  & \checkmark & $81.4$ & $80.5$ & $79.9$ & $35.8$ & \bm{$7.5$}\\
& & \checkmark &  & \checkmark & \checkmark & $82.1$ & $81.8$ & $81.5$ & $30.3$ & $9.3$\\
\cline{3-11}
& & \checkmark & \checkmark & \checkmark & \checkmark & \bm{$82.8$} & \bm{$82.4$} & \bm{$82.1$} & $29.9$ & $8.5$\\
\hline
\end{tabular}
\label{tbl:4featuresBadLink}
\end{table*}



%\begin{table*}[!t]
%\centering
%\begin{tabular} {|c|c|c|c|c|c|c|c|}
%\hline
%\multirow{2}{*}{\bf Links} & \multirow{2}{*}{\bf Featureset}         &   \multirow{2}{*}{\bf Reputation}      &    {\bf Precision}  &   {\bf Recall}  &  {\bf $F_1$-score} & {\bf FN} & {\bf FP}\\  
% &         &      &    {\bf (\%)}  &  {\bf (\%)}  & {\bf (\%)} & {\bf (\%)} & {\bf (\%)} \\  
%\hline
%$89,220$ 	& HTML  	& Trust	&   $67.5$ 	& $68.1$  	&  $67.7$	& $17.9$	& $14.0$\\
%\hline
%$89,220$ 	& HTML + JavaScript 	& Trust	&   $69.6$ 	& $70.4$  	&  $69.6$	& $18.4$ & ${\bf 11.3}$\\
%$89,220$ 	& HTML + ECDF 	& Trust	&   $72.8$ 	& $72.2$  	&  $72.4$	& $12.3$ & $15.5$\\
%$89,220$ 	& HTML + Topic 	& Trust	&   $71.8$ 	& $71.7$  	&  $71.7$	& $14.0$ & $14.3$\\
%\hline
%$89,220$ 	& HTML + JavaScript + ECDF 	& Trust	&  $74.4$ 	& $74.2$  	&  $74.3$ & $12.4$ & $13.4$\\
%$89,220$ 	& HTML + JavaScript + Topic 	& Trust	&   $73.3$ 	& $73.5$  	&  $73.4$ & $14.2$ & $12.3$\\
%$89,220$ 	& HTML + ECDF + Topic 	& Trust	&   $74.3$ 	& $73.6$  	&  $73.9$ & ${\bf 11.2}$ & $15.1$\\
%\hline
%$89,220$ 	& HTML + JavaScript + ECDF + Topic 	& Trust	&   ${\bf 75.5}$ 	& ${\bf 75.1 }$  	&  ${\bf 75.3 }$ & $11.3$ & $13.6$\\
%\hline
%\hline
%$84,714$ 	& HTML  	& Child safety	&   $68.9$ 	& $69.1$  	&  $69.0$	& $17.0$ & $13.9$\\
%\hline
%$84,714$ 	& HTML + JavaScript 	& Child safety	&   $71.7$ 	& $71.9$  	&  $71.6$	& $16.7$ & ${\bf 11.4}$ \\
%$84,714$ 	& HTML + ECDF 	& Child safety	&   $74.1$ 	& $73.4$  	&  $73.5$	& $10.5$ & $16.1$\\
%$84,714$ 	& HTML + Topic 	& Child safety	&   $74.6$ 	& $74.5$  	&  $74.6$	& $12.2$ & $13.3$\\
%\hline
%$84,714$ 	& HTML + JavaScript + ECDF 	& Child safety	&   $75.4$ 	& $74.9$  	&  $75.0$ & $10.4$ & $14.7$\\
%$84,714$ 	& HTML + JavaScript + Topic 	& Child safety	&   $76.1$ 	& $76.2$  	&  $76.2$ & $12.1$ & $11.7$\\
%$84,714$ 	& HTML + ECDF + Topic 	& Child safety	&   $76.2$ 	& $75.7$  	&  $75.9$ & ${\bf 10.1}$ & $14.1$\\
%\hline
%$84,714$ 	& HTML + JavaScript + ECDF + Topic 	& Child safety	&   ${\bf 77.5}$ 	& ${\bf 77.2}$  	&  ${\bf 77.3}$ & ${\bf 10.1}$ & $12.7$\\
%\hline
%\end{tabular}
%\caption{Opportunistic Predictive Performance using 5-fold cross validations while considering only bad embedded links for the ECDF features. Basic Classifier = Decision Tree.}
%\label{tbl:opportunistic}
%\end{table*}


==> structuralFeatures.tex <==
%!TEX root = ../submission.tex
\section{Prediction Using Structural Features}
\label{sec:structural}

\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{pics/system}
\caption{Overview of our classification framework. We crawl a larger
  number of web pages to extract structure- and content-based
  features. We also collect the available reputation ratings of the web
  pages through API calls to the WOT reputation system. We use these
  to train a predictive model, which is later used to predict the safety of a unknown web page. }
\label{fig:system}
\end{figure}


We use a {\em classification} approach, a well established supervised
learning-based algorithm~\cite{bishop07pattern}, to train a recognizer
for automatically determining the safety rating of web pages. Our
methodology relies on extracting suitable features that capture
properties of a web page. For {\em ground-truth} of web safety, we
rely on crowdsourced based reputation ratings of web pages, which we
obtain through API calls to the WOT reputation system.
Figure~\ref{fig:system} illustrates an overview of our classification
framework in general. Accordingly, we have developed a web crawler
that extracts different kinds of features and reputation ratings
(trustworthiness and child safety) for a large number of web pages and
stores the data in a database to be used by machine learning
algorithms for building a predictive model (recognizer). In the
following we describe our recognition framework, LookAhead, in detail.

\subsection{Structural Features of Web Pages}
\label{ssec:features}

A recognizer employing a supervised machine learning approach requires to perform a time consuming bootstrapping step before it can be deployed~\cite{bhattacharya14using}. A typical bootstrapping process involves obtaining suitable feature representation of the data and collecting a large amount of ground truth information. Often the feature extraction process is referred to as feature-engineering as it relies on domain-specific expertise. Moreover, the optimal feature-set is dependent on the target classes of interests and has been identified as a non-trivial problem~\cite{liu05toward}. 

\begin{table}[!t]
\centering
\caption{Prophiler performance on WOT dataset}
\begin{tabular} {|c|c|c|c|c|c|}
\hline
& {\bf Method}         &   {\bf FP\%}      &    {\bf FN\%}  & {\bf
  Reputation} & {\bf $F_1$-score \%}\\  
 &	(Feature sets)&	&  & {\bf Dimension} & \\
%& (Feature sets) & & & & \\
\hline
1 & Prophiler	&	$24.0$	&	$10.1$	& Trustworthiness & $66.6$\\
  & (HTML, JavaScript) & 	 &  & & \\
\hline
2 & Prophiler's top 3	&	$23.0$	&	$11.7$	& Trustworthiness & $65.1$ \\
  & (HTML, JavaScript) & 	 &  & & \\
\hline
3 & Prophiler's top 5	&	$23.2$	&	$12.6$	& Trustworthiness & $65.8$ \\
  & (HTML, JavaScript) & 	 &  & & \\
\hline
4 & Prophiler's top 75\% & $23.9$ & $10.2$ & Trustworthiness & $66.7$ \\
  & (HTML, JavaScript) & 	 &  & & \\
\hline
\hline
5 & Prophiler	&	$23.6$	&	$9.2$	& Child safety & $67.3$\\
  & (HTML, JavaScript) & 	 &  & & \\
\hline
6 & Prophiler's top 3	&	$21.6$	&	$11.4$	& Child safety & $67.3$ \\
  & (HTML, JavaScript) & 	 &  & & \\
\hline
7 & Prophiler's top 5	&	$23.9$	&	$10.2$	& Child safety
& $66.0$ \\
\hline
 & (HTML, JavaScript) & 	 &  & & \\
8 & Prophiler's top 75\% & $23.4$ & $9.3$ & Child safety & $67.4$ \\
  & (HTML, JavaScript) & 	 &  & & \\
\hline
\end{tabular}
\label{tbl:profilerOnWOT}
\end{table}



%Contrary to the state-of-the-art approaches, in this paper we propose the use of a novel set of features based on {\em empirical cumulative distribution function} (ECDF) and {\em topic modeling} to infer the safety of web pages. The main benefits of using ECDF and topic model based features are: (i) no requirement of domain knowledge to construct suitable feature representation of a web page and (ii) the features capture content related and thematic properties of a web page. Additionally, we show that the proposed novel features help to improve the recognition performance significantly (see Section~\ref{sec:results}).             

We use Prophiler~\cite{canali11prophiler} as the starting point. All
features used by Prophiler are ``static features'' in that they do not
require rendering the page or running any embedded code.  Among the
three feature sets used by Prophiler, we decided to leave out the set
of URL features because an overwhelming majority of the records in our
dataset (82\%) had less than half the URL features available. None had
all URL features available.  We describe the remaining two feature
sets below:
%% TODO Sourav to improve, or remove 


% Building on existing research, in this paper we first employ an opportunistic feature extraction technique that extracts features from the (i) HTML page structure and (ii) embedded Java Script code.
% %(iii) reputation scores of the embedded web links and (iv) text embedded in a web page to infer its safety. 
% Our method is opportunistic in the sense that not always all feature types are available and we handle this uncertainty by proposing a hierarchical classification technique. Details of our classification approach is given in Section~\ref{ssec:classifier}. Our feature extraction phase is done statically, i.e., we do not execute any code that is associated with a web page. The use of static features also help us to overcome long running time, cost, and scalability challenges often present in dynamic analysis-based approaches.


\subsubsection{HTML-based Features}
\label{sssec:html}
%Past years have seen a significant amount of effort in extracting an
%extensive number of features from the raw HTML content to detect if a
%web page is malicious. 
%In our work, we use the feature set proposed by Canali et
%al.~\cite{canali11prophiler}, which 
Prophiler uses a total of $19$ HTML-based features including the number
of {\em iframe} tags, the number of hidden elements, number of script
elements, the percentage of unknown tags, and number of malicious
patterns\footnote{Readers are referred to~\cite{canali11prophiler} for an
exhaustive and in-depth description of all the HTML features.}.    

\subsubsection{JavaScript-based Features}
\label{sssec:js}
Similarly to the HTML features, we adopt the exhaustive feature set of Canali et al.~\cite{canali11prophiler} in our analysis. $25$ JavaScript-based features are extracted by analyzing either the JavaScript file or the $<script>$ element embedded within the HTML text. Examples of JavaScript-based features include the number of times the {\em eval()} function is used, the number of occurrence  of the {\em setTimeout()} and {\em setInterval()} functions, the number of {\em DOM} modification functions, and the length of the script in characters (see~\cite{canali11prophiler}). % for in-depth description of the JavaScript features.  

\subsection{Classifier Training}
Our classification framework is adapted from Prophiler as well. Each
feature set uses its own classifier (C4.5 Decision Tree). The
results of the classifiers are combined using logical OR: i.e., if any
of the feature set classifier identifies a page as ``bad'', then the
classification framework declares the page as
``bad''. Figure~\ref{fig:prophiler-classifier} illustrates the
classification framework.

\begin{figure}[!t]
\centering
\includegraphics[width=0.6\linewidth]{pics/prophilerClassifier}
\caption{Classification framework for structural features, modeled
  after the Prophiler classification framework ($0 = $ good, $1 = $ bad).}
\label{fig:prophiler-classifier}
\end{figure}

\subsection{Results}
\label{ssec:profRes}
For our analysis, we selected all web pages in our dataset that (a)
have a rating in the corresponding WOT dimension and (b) have both
HTML and Javascript features available.  The resulting set has
$77,168$ pages with WOT trustworthiness ratings and $73,566$ pages
with WOT child safety rating (we defer a more detailed description of
our datasets to
Section~\ref{sssec:datasets}). Table~\ref{tbl:profilerOnWOT} shows the
results.

% Canali et al.~\cite{canali11prophiler} have reported very high
% accuracy, with false positive rate less than $1\%$ for $15,000$ web
% pages, while determining the potential maliciousness of web pages. 
% So,
% building on their work, we first applied the classification approach
% proposed by Canali et al. on the WOT dataset for trustworthiness and
% child safety, comprising respectively of $77,168$ and $73,566$ web
% pages (for detail description of the WOT dataset see
% Section~\ref{}). Results of this experiments are given in
% Table~\ref{tbl:profilerOnWOT}. 

From the table, we see that although the Prophiler classification
framework using HTML- and JavaScript-based feature sets was very
effective in detecting malicious web pages (Table~\ref{tbl:profiler}), its
generalizability is rather limited when the target application domain
is changed from detecting malicious web pages to detecting safety of
web pages in general. Both False Positives Rate (FP) and False Negatives
Rate (FN) increase significantly, resulting in $F_1$-scores of $66.6\%$ for
trustworthiness and $67.3\%$ for child safety.

One potential reason for this is the fact that HTML- and
JavaScript-based feature-sets only capture the structural properties
of web pages. They convey very little information regarding the
content of web pages. Thus, when trying to detect the content safety
of web pages, the structural feature set has limited
applicability. This shortcoming can be overcome by including features
that represent the content.  Motivated by this, in
Section~\ref{sec:content} we proceed to develop novel content-based
feature sets, which can perform better in predicting crowdsourced
reputation ratings for safety in general.

\noindent\textbf{A note on feature selection}: A smaller feature-set
is less expensive in terms of computation. The 
selection of features is therefore a tradeoff between cost and
classification performance.  Canali et al.~\cite{canali11prophiler}
considered how well smaller subsets of the Prophiler features perform,
compared to using all the features.  They tried the top-3 and top-5
features (Table~\ref{tbl:profiler}). We repeated this exercise as
well. We selected the top features as follows: using the correlation
score between an individual feature and the ground truth we ranked
features within a feature-set; We then selected the required number of
the top features for subsequent classification. The results are shown
in Table~\ref{tbl:profilerOnWOT} (rows 2-3 and 6-7).

We can observe the same patterns as in Table~\ref{tbl:profiler}: fewer
features result in better FP\% but a worse FN\%. The differences in the
classification
performance while using all the features vs using only the top-5
features are statistically significant (using McNemar Chi-squared test
with Yates' correction, $p \ll 0.01$) for both WOT dimensions.

Since a low FN\% is more important from the perspective of security,
we repeated the analysis considering the top 75\% HTML- and JavaScript
features. The results appear in row 4 and 8 of
Table~\ref{tbl:profilerOnWOT}. The classification performance while
using all the features is similar to that while using the top 75\%
features (the difference is not significant when tested using McNemar Chi-squared test
with Yates' correction at the confidence level of $95\%$). Therefore, for the
rest of this paper, we use the top 75\% HTML- and JavaScript features
for classification.

% Moreover, in order to see whether all the HTML- and Javascript
% features are essential (since more features implies greater complexity
% and processing cost), we
% we also carried out feature selection to pick the top $3$ and $5$
% features that correlate with the WOT ground-truth labels and also
% reported in the table above.
%Moreover, the use of identical HTML- and JavaScript-based features allows us to draw direct comparisons to the work of Canali et al., which we use as one of the baseline algorithms.





